Project 1640 Observations of the White Dwarf HD 114174 B

We present the first near infra-red spectrum of the faint white dwarf companion HD 114174 B, obtained with Project 1640. Our spectrum, covering the Y, J and H bands, combined with previous TRENDS photometry measurements, allows us to place further constraints on this companion. We suggest two possible scenarios; either this object is an old, low mass, cool H atmosphere white dwarf with Teff ~ 3800 K or a high mass white dwarf with Teff > 6000 K, potentially with an associated cool (Teff ~ 700 K) brown dwarf or debris disk resulting in an infra-red excess in the L band. We also provide an additional astrometry point for 2014 June 12 and use the modelled companion mass combined with the RV and direct imaging data to place constraints on the orbital parameters for this companion.

==> defn.tex <==
%-*-LaTeX-*-
% Copied from gmorris
% Note that some of these call others, eg \kmps uses \km.

% journals
\newcommand{\apj}{ApJ}
\newcommand{\mnras}{MNRAS}
\newcommand{\nat}{Nat}
\newcommand{\physrev}{Phys. Rev.}
\newcommand{\physrevB}{Phys. Rev. B}
\newcommand{\araa}{ARA\&A}                % "Ann. Rev. Astron. Astrophys."
\newcommand{\aap}{A\&A}                   % "Astron. Astrophys."
\newcommand{\aaps}{A\&AS}                 % "Astron. Astrophys. Suppl. Ser."
\newcommand{\aj}{AJ}                      % "Astron. J."
\newcommand{\apjs}{ApJS}                  % "Astrophys. J. Suppl. Ser."
\newcommand{\pasp}{PASP}                  % "Publ. Astron. Soc. Pac."
\newcommand{\apjl}{ApJ}                   % letter at ApJ
\newcommand{\pasj}{PASJ}
\newcommand{\gca}{Geochim. Cosmochim. Acta}
\newcommand{\physrep}{Phys. Rep.}
\newcommand{\aapr}{A\&A Rev.}
\newcommand{\procspie}{Proc. SPIE}
\newcommand{\memsai}{Mem. Societa Astronomica Italiana}
\newcommand{\pasa}{PASA}

% Length
\newcommand{\Mpc}{\rm\thinspace Mpc}
\newcommand{\kpc}{\rm\thinspace kpc}
\newcommand{\pc}{\rm\thinspace pc}
\newcommand{\AU}{\rm\thinspace AU}
\newcommand{\km}{\rm\thinspace km}
\newcommand{\mm}{\rm\thinspace mm}
\newcommand{\m}{\rm\thinspace m}
\newcommand{\cm}{\rm\thinspace cm}
\newcommand{\pix}{\rm\thinspace pixel}
\newcommand{\nm}{\rm\thinspace nm}
\newcommand{\micron}{\rm\thinspace $\mu$m}
%
\newcommand{\cmps}{\hbox{$\cm\s^{-1}\,$}}
\newcommand{\cmpssq}{\hbox{$\cm\s^{-2}\,$}}
\newcommand{\cmsq}{\hbox{$\cm^2\,$}}
\newcommand{\msq}{\hbox{$\m^2\,$}}
\newcommand{\mps}{\hbox{$\m\s^{-1}\,$}}
\newcommand{\cmcu}{\hbox{$\cm^3\,$}}
\newcommand{\pcmcuK}{\hbox{$\cm^{-3}\K\,$}}
\newcommand{\ppixsq}{\hbox{$\pix^{-2},$}}
\newcommand{\kpcsq}{\hbox{$\kpc^{2}\,$}}
% Length


% Time
\newcommand{\yr}{\rm\thinspace yr}
\newcommand{\Gyr}{\rm\thinspace Gyr}
\newcommand{\Myr}{\rm\thinspace Myr}
\newcommand{\s}{\rm\thinspace s}
\newcommand{\ks}{\rm\thinspace ks}
\newcommand{\ms}{\rm\thinspace ms}
\newcommand{\mus}{\hbox{$\mu\s\,$}}
\newcommand{\Ms}{\rm\thinspace Ms}
\newcommand{\hr}{\rm\thinspace hr}
% Time


% Frequency
\newcommand{\GHz}{\rm\thinspace GHz}
\newcommand{\MHz}{\rm\thinspace MHz}
\newcommand{\kHz}{\rm\thinspace kHz}
\newcommand{\Hz}{\rm\thinspace Hz}
% Frequency


% Temperature
\newcommand{\K}{\rm\thinspace K}
\newcommand{\C}{\rm\thinspace $^{\circ}$C}

% Temperature


% Pressure
\newcommand{\Kpcmc}{\hbox{$\K\cm^{-3}\,$}}
% Pressure


% Mass
\newcommand{\g}{\rm\thinspace g}
%
\newcommand{\gpcm}{\hbox{$\g\cm^{-3}\,$}}
\newcommand{\gpcmps}{\hbox{$\g\cm^{-3}\s^{-1}\,$}}
\newcommand{\gps}{\hbox{$\g\s^{-1}\,$}}
%
\newcommand{\Msun}{\hbox{$\rm\thinspace M_{\odot}$}}
\newcommand{\Msunpc}{\hbox{$\Msun\pc^{-3}\,$}}
\newcommand{\Msunpkpc}{\hbox{$\Msun\kpc^{-1}\,$}}
\newcommand{\Msunppc}{\hbox{$\Msun\pc^{-3}\,$}}
\newcommand{\Msunppcpyr}{\hbox{$\Msun\pc^{-3}\yr^{-1}\,$}}
\newcommand{\Msunpyr}{\hbox{$\Msun\yr^{-1}\,$}}
% Mass


% Energy
\newcommand{\MeV}{\rm\thinspace MeV}
\newcommand{\keV}{\rm\thinspace keV}
\newcommand{\eV}{\rm\thinspace eV}
\newcommand{\erg}{\rm\thinspace erg}
\newcommand{\Jy}{\rm\thinspace Jy}
\newcommand{\W}{\rm\thinspace W}
\newcommand{\mJy}{\rm\thinspace mJy}
%
\newcommand{\ergcmcups}{\hbox{$\erg\cm^3\ps\,$}}
\newcommand{\ergpcmps}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergpcmsq}{\hbox{$\erg\cm^{-2}\,$}}
\newcommand{\ergpcmcu}{\hbox{$\erg\cm^{-3}\,$}}
\newcommand{\ergpcmsqps}{\hbox{$\erg\cm^{-2}\s^{-1}\,$}}
\newcommand{\ergpcmsqpspA}{\hbox{$\erg\cm^{-2}\s^{-1}$\AA$^{-1}\,$}}
\newcommand{\ergpcmsqpspsr}{\hbox{$\erg\cm^{-2}\s^{-1}\sr^{-1}\,$}}
\newcommand{\ergpcmsqpsparcsecsq}{\hbox{$\erg\cm^{-2}\s^{-1}\mathrm{arcsec}^{-2}\,$}}
\newcommand{\ergpcmcups}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergps}{\hbox{$\erg\s^{-1}\,$}}
\newcommand{\ergpssq}{\hbox{$\erg\s^{-2}\,$}}
\newcommand{\ergpspmp}{\hbox{$\erg\s^{-1}\Mpc^{-3}\,$}}
\newcommand{\ergpspkpc}{\hbox{$\erg\s^{-1}\kpc^{-1}\,$}}
%
\newcommand{\keVpcmsqpspsr}{\hbox{$\keV\cm^{-2}\s^{-1}\sr^{-1}\,$}}
%
\newcommand{\WpHzpsr}{\hbox{$\W\pHz\psr\,$}}
% Energy

% X-ray observations
\newcommand{\cts}{\rm\thinspace ct}
\newcommand{\ctsps}{\hbox{$\cts\s^{-1}\,$}}
% X-ray observations

% Ionisation Parameter
\newcommand{\ergcmps}{\hbox{$\erg\cm\ps\,$}}
% Ionisation Parameter

% Force
\newcommand{\dyn}{\rm\thinspace dyn}
\newcommand{\dynpcmsq}{\hbox{$\dyn\cm^{-2}\,$}}
% Force


% Speed
\newcommand{\kmps}{\hbox{$\km\s^{-1}\,$}}
\newcommand{\kmph}{\hbox{$\km\hr^{-1}\,$}}
\newcommand{\kmpspmp}{\hbox{$\km\s^{-1}\Mpc^{-1}\,$}}
\newcommand{\kmpspMpc}{\hbox{$\kmps\Mpc^{-1}\,$}}
% Speed


% Luminosity
\newcommand{\Lsun}{\hbox{$\rm\thinspace L_{\odot}$}}
\newcommand{\Lsunppc}{\hbox{$\Lsun\pc^{-3}\,$}}
% Luminosity


% Misc
\newcommand{\plawnorm}{\hbox{$\rm\thinspace photons\keV^{-1}\cm^{-2}\s^{-1}\,$}}
\newcommand{\Zsun}{\hbox{$\thinspace \mathrm{Z}_{\odot}$}}

\newcommand{\gauss}{\rm\thinspace gauss}
%
\newcommand{\chisq}{\hbox{$\chi^2$}}
\newcommand{\delchi}{\hbox{$\Delta\chi$}}
%
\newcommand{\ph}{\rm\thinspace ph}
% Misc

% Angles
\newcommand{\amin}{\rm\thinspace arcmin}
\newcommand{\aminsq}{\hbox{$\amin^{2}\,$}}
\newcommand{\asec}{\rm\thinspace arcsec}
\newcommand{\masec}{\rm\thinspace milli-arcsec}
\newcommand{\masecppx}{\rm\thinspace milli-arcsec/pixel}
\newcommand{\asecsq}{\hbox{$\asec^{2}\,$}}
\newcommand{\sr}{\rm\thinspace sr}
\newcommand{\degword}{\rm\thinspace deg}
\newcommand{\degsym}{\rm$^{\circ}$}
\newcommand{\degsq}{\hbox{$\degword^2\,$}}
% Angles

% Emission measure
\newcommand{\emm}{\hbox{$\cm^{-5}\,$}}
\newcommand{\empasecsq}{\hbox{$\emm\asec^{-2}\,$}}
\newcommand{\keVempasecsq}{\hbox{$\keV\emm\asec^{-2}\,$}}
% Emission measure

% Per something
\newcommand{\pcm}{\hbox{$\cm^{-1}\,$}}
\newcommand{\psqcm}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pcmsq}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pcmcu}{\hbox{$\cm^{-3}\,$}}
\newcommand{\pmpc}{\hbox{$\Mpc^{-1}\,$}}
\newcommand{\pmpccu}{\hbox{$\Mpc^{-3}\,$}}
\newcommand{\ps}{\hbox{$\s^{-1}\,$}}
\newcommand{\pHz}{\hbox{$\Hz^{-1}\,$}}
\newcommand{\pcmK}{\hbox{$\cm^{-3}\K$}}
\newcommand{\phpcmsqps}{\hbox{$\ph\cm^{-2}\s^{-1}\,$}}
\newcommand{\psr}{\hbox{$\sr^{-1}\,$}}
% Per something

%Frame rates
\newcommand{\fps}{\rm\thinspace fps}
\newcommand{\MB}{\rm\thinspace MB}
\newcommand{\MBps}{\rm\thinspace MB/s}

%GR
\newcommand{\rg}{\rm\thinspace $r_\mathrm{g}$}

% misc
% \newcommand{\texttilde}{${}_{\textrm{\symbol{126}}}$}


%cosmology

%cosmology

% Use times for maths fonts
% \DeclareSymbolFont{operators}   {OT1}{ptmcm}{m}{n}
% \DeclareSymbolFont{letters}     {OML}{ptmcm}{m}{it}
% \SetMathAlphabet{\mathbf}{normal}{\encodingdefault}{\rmdefault}{\bfdefault}{n}%
% \SetMathAlphabet{\mathsf}{normal}{\encodingdefault}{\sfdefault}{m}{n}%
% \SetMathAlphabet{\mathrm}{normal}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetSymbolFont{operators}{bold}{OT1}{ptmcm}{b}{n}
% \SetSymbolFont{letters}{bold}{OML}{ptmcm}{b}{it}
% \SetMathAlphabet{\mathbf}{bold}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetMathAlphabet{\mathsf}{bold}{\encodingdefault}{\sfdefault}{b}{n}%
% \SetMathAlphabet{\mathrm}{bold}{\encodingdefault}{\rmdefault}{b}{n}%

%\thinmuskip=2.5mu
%\medmuskip=3.5mu plus 1mu minus 1mu
%\thickmuskip=4.5mu plus 1.5mu minus 1mu
%\DeclareSymbolFont{symbols}     {OMS}{cmsy}{m}{n}
%\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
%\SetSymbolFont{symbols}{bold}{OMS}{cmsy}{b}{n}
%\SetSymbolFont{largesymbols}{bold}{OMX}{cmex}{m}{n}

